Information Flow Control in Machine Learning through Modular Model Architecture

In today's machine learning (ML) models, any part of the training data can affect the model output. This lack of control for information flow from training data to model output is a major obstacle in training models on sensitive data when access control only allows individual users to access a subset of data. To enable secure machine learning for access-controlled data, we propose the notion of information flow control for machine learning, and develop an extension to the Transformer language model architecture that strictly adheres to the IFC definition we propose. Our architecture controls information flow by limiting the influence of training data from each security domain to a single expert module, and only enables a subset of experts at inference time based on the access control policy.The evaluation using large text and code datasets show that our proposed parametric IFC architecture has minimal (1.9%) performance overhead and can significantly improve model accuracy (by 38% for the text dataset, and between 44%--62% for the code datasets) by enabling training on access-controlled data.

==> background.tex <==
\section{Motivation for IFC in ML}
\label{sec:use-cases}
The capability to control information flow from training data to model outputs is important in many use cases, where different users can only access different subsets of the training data. Below, we briefly discuss example use cases. 

% \subsection{Example Use Cases}
% \hl{[Ed] Provide a broader high-level discussion - there are many cases where different users have different access permissions for subsets of training data: code repository, documents, military, etc. Then provide more in-depth discussions on a few examples.

% I wrote down a few examples that I think can be compelling. They are placeholders and need to be propertly written.
% }  

\noindent {\bf Writing Assistant for Internal Documents.}
A language model can be used to provide text suggestions when writing documents with sensitive content, such as company internal memos, project reports, military documents, etc. 
The language model can perform better if it can leverage related (sensitive) content that the user has access to.
For instance, when writing a project report, the language model accessing other documents from the same project will provide more tailored suggestions. However, we need to ensure that the model's suggestions do not leak any information from other inaccessible documents.

% \hl{Can add reddit type example here to movitvate our Reddit evaluation. Say reddit simulates different working groups in this example}

\noindent {\bf AI Coding Assistant.}
In order to provide more relevant suggestions, a code completion model for coding assistant can be trained using code from a company's internal repositories.
However, code repositories typically have access control, and individual engineers only have access to a subset of repositories.
A code completion model needs to honor the access restrictions and only suggest code based on the repositories that a particular user has access to at inference time.   

% Language model (LM) Trained using code from access controlled repositories -- different users have access to a subset of repositories. Generated code for each users should only depend on accessible repositories.
%
% Or training code with different licenses -- a user needs to be able to specify which types of licenses may be used for his/her code.



% documents that a particular user has access to such as other documents in Google Drive. But the model outputs should only depend on the documents that each user has access to.

% %%%%%%%%%%%%%% META DELETE %%%%%%%%%%%%%
% \noindent {\bf Generative AI with Copyrighted Training Data.}
% While we only evaluate Language Models in this work, the IFC concept can be extended to other types of machine learning models. 
% For instance, consider a service that allows users to generate images using a generative image model that is trained using copyrighted work from many artists while charging individual users for the right to generate images based on a particular artist's work.
% In this scenario, each user has the rights to use a different combination of artists' work depending which ones they paid for.
% Therefore, the image generation model needs to be able to control which training data (artists' work) can affect its outputs depending on each user's access permissions. A similar scenario can also apply for other types of generative AI models such as language models to generate text and models to generate music/sound.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%However, other users might not have the rights to said art and therefore the model must not use that data when generating output for them. Here again, there can be several artists providing copyrighted work, and several users willing to pay for any given (combination) of artists. 

% Imagine the case where a user needs to pay extra money in order to a certain artist's pictures in image generation model. Each user has a different set of images that can be used for a generative AI model. The model output should only depend on the images that each user has a right to use.


\noindent {\bf AI-based Q/A on Access Controlled Materials.}
The recent advances in large language models (LLMs) showed a potential in search or Q/A engines (e.g., ChatGPT, Bing Chat). 
While these models are only trained on public domain data today, it is likely that the LLM-based search or Q/A engines will also be applied to answer questions based on access controlled data such as pay-walled content (e.g., Wall Street Journal, New York Times, etc), internal corporate documents, etc.  
In such cases, the LLM may need to be fine-tuned with the access controlled data for the best performance.
However, in order to prevent unintended leakage of access controlled data, the fine-tuned model should be able to ensure that its output only depends on the subset of the training data that a particular user is allowed to access.

% \begin{enumerate}
    %\paragraph*{\textbf{Licensed datasets in generative AI}} 
    %Today, we have many generative AI models---DALL.E 2~\cite{ramesh2022hierarchical}, GPT~\cite{radford2018improving} (and its successors like GPT-2, 3 and ChatGPT). The issue with these types of models is that they often are limited to be trained only on public domain data since we cannot guarantee that if trained on licensed or pay-walled data, then this data will not be reflected into the output. However, it's conceivable that users who might have purchased the ability to access such data be able to benefit from that data through its use in the ML model. For instance, there have been many discussions on using ChatGPT as a Question Answer (Q/A) engine. However, to be more effective at this, ChatGPT would benefit from high quality information sources. Unfortunately, many of these information sources (e.g., Wall Street Journal, New York Times, etc) tend to be pay-walled. However, if a given user does have access to some of these sources, then it would be ideal if the model can utilize this additional data for the output. This gives rise to the following problem---if there are a large number of users, each different subsets of accessible resources, how does a model guarantee that each user can benefit from the subset of resources they paid to have access to, but doesn't leak information from the resources they do not have access to? 
    %Aside from language models, this can also apply to generative vision models that create artwork. Again, there might be some users who purchased copyrights to art from artists and would like it to be used by the model to create the output artwork. However, other users might not have the rights to said art and therefore the model must not that data when generating the output. 
    
    %\paragraph*{\textbf{Sensitive datasets in generative AI}}
    %Aside from licensed/pay-walled data, there are certain datasets that are sensitive in nature, and therefore not everyone who uses the final model might have access to these sensitive datasets. For instance, one could imagine automated Q/A systems using customer information---not all users of the Q/A systems would have access to all the customer data that was used to train it, and so the model has to guarantee that the model can provide output leveraging customer data they have access to while preventing leakage from data they do not have access to. The same goes with code auto-completion frameworks like GitHub Copilot. While Copilot is trained only on public code, other code auto-completion models could potentially be trained different code bases that are each accessible only by a subset of users. In such a case, how does one have a model that guarantees no leakage to users without access to those code bases, but also using the sensitive code bases for those users that do?




\section{Background and Related Work}
\label{sec:background}

In this section, we discuss relevant backgrounds: Transformer-based language models, and IFC, and NI. 
%We first describe the Transformer-based language model, which is the main target of this paper. 
% and the Mixture-of-Expert (MoE) models, which we leverage to develop our protection scheme.
%Then, we briefly define the traditional notion of non-interference, which we use to develop the corresponding notion for information flow control in machine learning (ML).

\subsection{Language Modeling and Transformers}
%One of the goals of Natural Language Processing (NLP) is to learn the joint probability function of sequences of words in a language~\cite{bengio2000neural}.
This paper focuses on generative language modeling, which relies heavily on next token prediction---the task of predicting the next most probable \emph{token} for any given sequence of tokens. For language modeling, the accuracy is measured with \emph{perplexity}, an exponentiation of the negative log likelihood of the text. Lower perplexity implies better performance. 

% \hl{
% FIGURE - Transformer architecture. Need to show enough details so that the readers can understand different architecture options (MLP, adaptor, etc.) later.
% }

\begin{figure}
    \centering
\includegraphics{images/transformer.pdf}
\vspace{-0.10in}
    \caption{\small Generic transformer architecture}
    \label{fig:transformer}
\vspace{-0.2in}
\end{figure}

The current state-of-the-art language models use Transformers~\cite{vaswani2017attention, radford2018improving,devlin2018bert,yang2019xlnet,liu2019roberta,raffel2020exploring,zhang2022opt,black2022gpt}. %Many researchers have released various high-performing Transformers~\cite{radford2018improving,devlin2018bert,yang2019xlnet,liu2019roberta,raffel2020exploring,zhang2022opt,black2022gpt}.
At the highest level, Transformers (shown in Figure~\ref{fig:transformer})take a sequence of tokens as input, pass it through several encoder and decoder layers, to produce an output a probability distribution over the next possible token (in the case of the language modeling objective). These Encoder/Decoder blocks may themselves have ``attention''~\cite{vaswani2017attention} and feedforward layers. The resulting output distribution is compared to the ground truth, and cross-entropy loss is computed to measure the quality of the prediction. 

% Figure~\ref{fig:transformer} shows a popular Transformer model, GPT-$2$~\cite{radford2018improving}.
% %
% GPT-$2$ is a decoder-only Transformer model, which takes in input texts converted to a vector representing the sequence of  thetokens. This vectorized input is passed through GPT-$2$'s two embedding layers, followed by $12$ Transformer blocks and a normalization layer (Figure~\ref{fig:transformer}). Each of the $12$ Transformer blocks consist of $2$ attention layers and $1$ MLP layer, interspersed with normalization layers. 
%These attention layers are the hallmark of Transformers, and allow GPT-$2$ to pay attention to specific, important parts of the token vector. 
%This work amends this architecture of GPT-$2$ to have experts per security domain and add a gating function that allows us to route any user input to specific experts based on the access policy of the user, and the relevance of the expert to the input at hand. 
% This work is mainly evaluted on a modified GPT-$2$ model; however, our proposed idea is generally applicable to other Transformer models as well.
% \textcolor{red}{Kiwan: Now we have OPT as well. Do we need to explain or mention its internals?} \trishita{Perhaps we can remove this and show a more general transformer architecture? Just to make the paper not look too GPT-2 specific?}

\subsection{Traditional Non-Interference (NI)}
\label{sec:ni}
Non-Interference~\cite{goguen1982security} is a security policy commonly used in information flow control to limit the influence between security levels. Let $D$ represent the machine state, and let $d_L$ and $d_H$ be the projection of the machine state $D$ to the low sensitivity and high sensitivity parts, respectively. Let $=_L$ be the function that compares the low sensitivity parts of the state, i.e., $D =_L D^{\prime}$ iff $d_L =_L d_L^{\prime}$. Let $(P, D_{t1}) \rightarrow^* D_{t2}$ be the execution of the program $P$ starting with machine state $D_{t1}$ and terminating with the machine state $D_{t2}$. Given this, we define Non-Interference for a deterministic program $P$ as follows~\cite{goguen1982security}:
\begin{align*}
    \forall D_{t1}, D_{t1}^{\prime} : D_{t1} &=_L D_{t1}^{\prime} \wedge \\
    (P, D_{t1}) &\rightarrow^* D_{t2} \wedge \\
    (P, D_{t1}^{\prime}) &\rightarrow^* D_{t2}^{\prime} \Rightarrow \\
    D_{t2} &=_L D_{t2}^{\prime}
\end{align*}
In other words, a deterministic program $P$ satisfies Non-Interference if, given the same initial low sensitivity machine state, its transformation of the low sensitivity machine state is the same regardless of the high sensitivity machine state.

% Non Interference is a strict policy, however, it holds only when $P$ is deterministic. For randomized algorithms, we use Differential Privacy, as defined below.

%\subsection{\textbf{Differential Privacy}}
%Differential Privacy (DP) is a system for sharing information about a dataset by describing the patterns of groups within the dataset without leaking infromation about individuals in the dataset. One of the most popular mathematical definitions of DP is $\epsilon$-DP, defined below.
%
%\paragraph*{\textbf{$\epsilon$-Differential Privacy}}
%Let $\epsilon \in \mathbb{R}_{\geq 0}$ and a $\mathcal{A}$ be a randomized algorithm that takes a dataset as input. Let $O$ denote all possible outputs of $\mc{A}$. The algorithm $\mc{A}$ is said to provide $\epsilon$-Differential Privacy if, for all datasets $D_1$ and $D_2$ that differ on a single element:
%\begin{equation*}
%e^{-\epsilon} \leq \frac{P(\mc{A}(D_1) \in O)}{P(\mc{A}(D_2) \in O)} \leq e^{\epsilon}
%\end{equation*}
%where the probability is taken over the randomness in $\mc{A}$
%
%In other words, enforcing DP guarantees that the output of a randomized algorithm (like many ML models) on two datasets that differ by a single data point is within a small threshold of $e^\epsilon$.



% \subsection{Mixture-of-Experts (MoE) Models}

% % \hl{
% % FIGURE - MoE architecture. Need to clearly show multiple parallel/independent sub-models and the gating function.
% % }

% \begin{figure}
%     \centering\includegraphics{images/moe.pdf}
% \vspace{-0.1in}
%     \caption{\small Mixture of Experts architechture}
%     \label{fig:moe}
% \vspace{-0.25in}
% \end{figure}

% Mixture of Experts (MoE) refers to a ML technique where, instead of one large network, multiple smaller networks called \emph{experts} divide a given problem space into multiple regions~\cite{masoudnia2014mixture}. 
% As shown in Figure~\ref{fig:moe}, each expert is a set of layers within the larger model, and different experts are stacked in parallel to each other. There is typically a \emph{gating function} which, at inference time, decides which of the experts should be activated for a given input. Once this decision is made, the input is then passed through the selected experts, and their outputs are aggregated at the end to produce one final output. 
% There are several different ways of implementing the gating function, which we broadly categorize into two: 

% %\begin{enumerate}
%     %\item 
%     \noindent {\bf Learned Routing.} One of the most popular approaches is to train the gating function together with all experts, therefore letting the gating function learn which experts to activate for which input during training. While such an approach can be made fast at inference~\cite{shazeer2017outrageously,lepikhin2021gshard,dathathri2020plug,chen2022mod}, it is not flexible; we have to re-train the entire gating function (and thus the entire model) if we want to add/remove/modify any of the experts. Furthermore, since the gating function is trained together with data from all domains, it's internal state is a mix of all domains. Thus, at inference, it is difficult to isolate and remove the influence of inaccessible domains and ensure that the gating function is secure.
%     % They also do not provide any information flow control guarantees 
    
%     \noindent {\bf Deterministic Routing.} In order to address the lack of flexibility in terms of expert modfication, Gururangan et.al. proposed DeMix~\cite{gururangan2021demix}, where they leverage conditional language modeling to remove the need for training the gating function, thereby granting the ability to add, remove, or modify experts ad hoc to the otherwise static MoE architecture. However, this comes at the expense of scalability, since DeMix requires \emph{all} experts to process each input before it appropriately weighs the outputs of these experts and combines them to produce one final output.
    
% %\end{enumerate}
% In this work, we need both the flexibility of modifying experts on-the-fly and the scalability to support a large number of domains. We provide details for how we construct a gating function satisfying these properties in Section~\ref{sec:ifc-nlp}.

==> discussion.tex <==
\section{Discussion}
%\section{Naive Solutions vs Our Approach}

\trishita{this would be a good place to mention RAG?}
We now discuss a few simple solutions and highlight why they are either insufficient from a security perspective, or infeasible from a practical standpoint. We then describe how our approach satisfies both the security requirements outlined in Sections~\ref{sec:prob-statement} and ~\ref{sec:operationalization}, and the practical considerations in Section~\ref{sec:prac-considerations}.

\noindent {\bf Train Only on Public Data.} For security, one naive option is to use a model pre-trained only on public data. Because this model is not trained with any access controlled data, it cannot leak information from the security domains. However, these pre-trained models are known to be too general and cannot perform specific tasks as well as fine-tuned models. As an example, Figure~\ref{fig:baseline} shows the perplexity (the measure of accuracy, lower is better) of GPT-2 on $50$ different datasets (security domains) from Pushshift.io. The GPT-2 model that is fine-tuned on these Pushshift.io domains significantly outperforms the same GPT-2 model with only pre-training.
This result clearly shows the benefit of fine-tuning a model with additional in-domain data for accuracy ({\bf G1}; see Section~\ref{sec:evaluation} for details).

\begin{figure} 
\begin{center}
\includegraphics[]{baseline.pdf}
\vspace{-0.2in}
\caption{\small Pre-trained GPT-$2$ evaluated on $50$ datasets from Pushshift.io consistently underperforms GPT-$2$ fine-tuned on all $50$ datasets. \label{fig:baseline}}
% Domains $51-58$ are \emph{unseen} domains, i.e., domains that were not included in the training of the fine-tuned  model.
% \hl{annotate the unseen rather than mark them with a separate dot}
\end{center}
\vspace{-0.275in}
\end{figure}

%\paragraph*{\textbf{Fine-tuning with all data}} Another option is to ignore the access policy restrictions and simply fine-tune a single model on data from all $m$ security domains. While this will likely outperform a model that is not trained with this data, it violates our definition of \textbf{$\epsilon$-NI}.

\noindent {\bf Fine-tune One Model for Each Combination of Security Domains.} 
Another secure option is to fine-tune a new model for each possible combination of security domains. Unfortunately, for $m$ domains, this approach requires fine-tuning $2^m$ different models. 
The exponential number of models suggests that this approach will not be practical unless $m$ is very small
(\textbf{G3.1}).

\noindent {\bf Fine-tune One Model for Each Security Domain.} 
Another option is to fine-tune one model for each security domain, and choose one model that a user has access to at run-time. 
This approach reduces the total number of models needed to be fine-tuned from $2^m$ to $m$. 
However, our experimental results later show that this approach is sub-optimal and a user with access to multiple domains can significantly improve a model's output quality (higher accuracy) by using multiple domains at the same time. 
%
%Ensembling more than one experts is nontrivial as gating 
%Given that fine-tuning a separate model for each \emph{combination} of security domains is prohibitively expensive, another option is to simply to fine-tune one model for each security domain, and simply use one model that is most relevant to the user's input but is also permitted by the access policy of that user. This would bring down the total number of models needed to be fine-tuned from $2^m$ to $m$, and thus is much cheaper. However, as we will see in Figure~\ref{fig:ablate-k-pol} in Section~\ref{sec:ablation}, there is often a benefit of using more models that has seen more data than just a single domain. This is because text can sometimes naturally span multiple domains---e.g., text related to Bitcoin would be similar to both technology related text, as well as finance related text, and thus when evaluating such text it would be beneficial to use a model that has seen both types of text. Furthermore, we also see (and will later discuss) in Figure~\ref{fig:ablate-k-pol}, when there are a very few and suboptimal domains that are accessible to a user, it is better to use the data from all the domains combined than to use just a single domains.

% Another option is to fine-tune a new model on data from each possible combination of security domains. Thus, for $m$ domains, this would mean fine-tuning $2^m$ different models. Given the exponential number of models, as $m$ increases, this solution will take up too much compute, memory and storage for training and storing all the models. It is easy to see that such a solution will not scale for a large number as it will violate \textbf{G3.1}.

%\paragraph*{\textbf{Existing Mixture of Experts}}
% (see also Table~\ref{tab:rel-work})
%One possiblity is to leverage Mixture of Experts (MoE) architechtures in order to achieve our security properties. We could implement this by training one expert for each security domain, and then, at inference, only activate the experts the end user has access to and appropriately combine the experts' outputs to produce one final output. While, at a high-level, this approach seems viable, there are a few reasons why off-the-shelf MoE solutions are not well suited for our purposes:
%\begin{enumerate}
%    \item \textbf{No Access Control}: Existing MoE solutions have gating functions that cannot provide any strict guarantees on how information is used from each expert towards the final output, violating \textbf{$\epsilon$-NI}. 
%    \item \textbf{Modularity or Scalability}:
%    As discussed in Section~\ref{sec:background}, gating functions in existing MoE fall into two categories: trained and untrained. Trained gating functions can be \emph{scaled} (\textbf{G3}) to include a large number of experts~\cite{shazeer2017outrageously}, whereas untrained gating functions are designed to be \emph{modular} (\textbf{G2}) to allow the addition or removal of experts without retraining the entire model~\cite{gururangan2021demix}. However, as we've seen in the prior discussion one property always comes at the expense of the other, thus either violating \textbf{G2} or \textbf{G3}. Hence, we will need to overhaul these gating functions to accommodate both.  
%\end{enumerate}
%Table~\ref{tab:rel-work} also concisely summarizes the reasons why other state-of-the-art MoE solutions cannot be used for the purposes of this work.

%\begin{table}
%\centering
%\begin{tabular}{ c c c c}
%& \thead{Modularity} & \thead{Access \\ Control} & \thead{Scalability} \\ 
% Mod-Squad~\cite{chen2022mod} & \xmark & \xmark & \cmark \\
% % Input Partitioning~\cite{tang2002input} & \xmark & \xmark & \xmark \\
% Sparsely-Gated MoE~\cite{shazeer2017outrageously} & \xmark & \xmark & \cmark \\
% GShard~\cite{lepikhin2021gshard} & \xmark & \xmark & \cmark \\
% PPLM~\cite{dathathri2020plug} & N/A & \xmark & \cmark \\
% % CTRL~\cite{keskar2019ctrl} & \xmark & \xmark & \xmark \\
% DExperts~\cite{liu2021-dexperts} & \cmark & \xmark & \xmark \\
% Demix~\cite{gururangan2021demix} & \cmark & \xmark & \xmark \\ 
%\end{tabular}
%\caption{\label{tab:rel-work} \small All existing approaches for Mixture of Experts are not made for information flow control, and thus lack one or more of the necessary qualities for a viable solution}
%\end{table}

% \vspace{-0.1in}
\subsection{Our Approach: Parametric NI for Transformers}
Our approach to parametric NI involves separately training different experts with data from each security domain to ensure parametric isolation. Then, at run-time, once we have the user's input and access-policy, we them in our gating algorithms to calculate the top-$k$ experts that permitted by the access policy, and are likely to be best suited for the user's input. Finally, once we have our top-$k$ expert models, we then use them in our ensembling schemes to produce one final output for the user. Each of these steps is carefully designed to ensure no information is leaked from domains that are not allowed by the access policy. Here is how our approach fulfills the various requirements needed for a secure and practical implementation of parametric NI: 
% \trishita{TODO: very briefly explain our approach so the discussion below makes sense. No need for details at this point since overview section is right after this}
% In order to control the influence of training data on model outputs in a scalable and effective manner, we propose a few modifications that can be incorporated into existing, off-the-shelf transformer architectures. Intuitively, we separately train a small subset of the parameters of the parent transformer model, one separate copy for each of the $m$ security domains. This is done to achieve parametric isolation of each of the security domains, and there are several different approaches to accomplish this~\cite{masoudnia2014mixture, hu2021lora, houlsby2019parameter}, which will be briefly described in Section~\ref{sec:exp-arch}. At the inference time, our gating function activates only $k$ out of $m$ experts based on access permissions and relevance to the user's input. 
% The relevance of the current user input to the experts must be done in a way that does not use any information from the inaccessible experts. Since which experts are inaccessible are dictated by the access policy, which is only available at run-time, we are limited in the amount of offline computation we can leverage to determine expert relevance as we need to ensure the ranking process does not leak information from experts that might be inaccessible. This thus presents us with unique design challenges, since we must now construct a gating scheme that is fast, incorporates expert access restrictions, scales to a large number of experts, and provides relevant matches with limited user input at run-time.
% This, to the best of our knowledge, has not been explored before, and thus presents a unique design challenge that we examine in Sections~\ref{sec:gate-k} and~\ref{sec:gate-unk}. Then, the overall model output is determined by running the user input through a final model that is a combination of the $k$ expert parameters, or ensembling the outputs of the $k$ activated experts after providing the input to each of them separately. 
% While, at a glance, this approach may appear similar to today's off-the-shelf MoE models, the MoE architecture needs to be significantly modified to ensure non-interference while meeting the practical design goals G$1$, G$2$, and G$3$.

%\begin{itemize}[leftmargin=*]
%\item 
\noindent {\bf Security (Non-interference).} The traditional transformer architecture cannot ensure non-interference chiefly because it does not have mechanisms to enforce parametric isolation to ensure that parameters from training on sensitive data from different security domains are kept separate. Because of this, these traditional models also cannot honor any access policy that prohibit use of certain data at inference. 
% This is because, for non-interference, the model's gating function should only use information from accessible domains, so that it can prevent information flow from the experts deemed inaccessible by the access policy provided at inference. 
% In today's MoE or other ensemble models, this is not the case because the gating function is often trained using data from all domains, and therefore its internal state cannot isolate the inaccessible domains at inference. 
We eliminate the information leakage through gating functions by designing our gating function such that the internal state for each domain is kept separately. 
    % is a conglomeration of data from all domains, and it therefore cannot isolate 

% , thereby guaranteeing no information leakage from them
%\item 
\noindent {\bf Scalability (G3) and Modularity (G2).} The traditional MoE architecture typically has a relatively small number of fixed experts. To allow scalability to a large number of security domains, we carefully design the expert model architecture so that each expert has a relatively small number of parameters. For the same reason, we also design our gating function such that out of all the accessible experts, it activates only the top-$k$ most relevant experts. Finally, to support dynamic changes in security domains, the gating and ensembling decisions are designed to be made quickly and without re-training.
% , which is also hard to do with the traditional MoE architecture, as discussed in Section~\ref{sec:background}.

%\item 
\noindent {\bf Accuracy (G1).} The security, modularity, and scalability constraints significantly limit the information that can be used to make gating/ensembling decisions, the size of each expert, and the number of experts that can be activated ($k$). It is a significant challenge to achieve high accuracy under this constrained environment. We show that our proposed design can significantly improve the accuracy compared to a pre-trained model. 
    % \hl{We need to highlight why we do top-$k$, because we spend a fair amount time discussing how to pick the top-k experts, but do not discuss why we only limit ourselves to $k$}
%\end{itemize}
% The secure MoE model for information flow control needs to address new technical challenges in order to provide both security and efficiency at the same time. 

% \begin{itemize}

% \item {\bf Security (non-interference)}: For non-interference, the model needs to decide which experts to activate and what the ensemble weights should be {\em only using information from accessible domains}. In today's MoE or other ensemble models, these decisions leak information because they use data from all domains, often through a learning-based approach. 
%This implies that the MoE gating function or ensemble weights cannot be obtained by training a model using all the data, which is a typical approach in today's MoE models.
    
% \item {\bf Modularity (G2) and scalability (G3)}: The traditional MoE architecture typically has a relatively small number of fixed expert domains. To support a large number of security domains, each expert model needs to have a relatively small number of parameters. Also, to support dynamic changes in security domains, the gating and ensemble decisions must be made quickly and without re-training. 


%In order to obtain the optimal accuracy for any given input, our gating function computes, then activates only the top $k$ accessible+relevant experts, out of all $m$ experts. This utilizing irrelevant experts pollutes the final output with noise, thus reducing accuracy (See Section~\ref{sec:ablation}). % cite top k
% In fact, we found that activating too many experts unnecessarily can also hurt the accuracy (See Section~\ref{sec:ablation}). % cite top k

%\item [G2]: To preserve modularity, we use a gating function that does not need to be trained. With this, each of the experts can be trained asynchronously and individually, and can be easily added and removed from the overall model later.

%\item [G3]: In order to make our model scalable for a large $m$, at inference, we formulate a gating function that is able to pick which experts are relevant to the user's input without having to evaluate said input on all experts. Furthermore, we truncate the list of relevant experts to only the top-$k$ experts, thereby allowing us to save resources by evaluating our input on fewer experts. 

% \end{itemize}



